Learning to Write on Dirty Paper

Dirty paper coding (DPC) is a classical problem in information theory that considers communication in the presence of channel state known only at the transmitter. While the theoretical impact of DPC has been substantial, practical realizations of DPC, such as Tomlinson-Harashima precoding (THP) or lattice-based schemes, often rely on specific modeling assumptions about the input, state and channel. In this work, we explore whether modern learning-based approaches can offer a complementary path forward by revisiting the DPC problem. We propose a data-driven solution in which both the encoder and decoder are parameterized by neural networks. Our proposed model operates without prior knowledge of the state (also referred to as "interference"), channel or input statistics, and recovers nonlinear mappings that yield effective interference pre-cancellation. To the best of our knowledge, this is the first interpretable proof-of-concept demonstrating that learning-based DPC schemes can recover characteristic features of well-established solutions, such as THP and lattice-based precoding, and outperform them in several regimes.

==> common.tex <==
% Utility file


\usepackage{amsmath,amssymb,amsfonts,bbm,bm,mathrsfs}
\usepackage{color}
\usepackage{algorithmic}
\usepackage{graphicx}
\usepackage{textcomp}
\usepackage{xcolor}
% \usepackage{hyperref}
\usepackage{amsthm}

% \usepackage{flushend}

\usepackage[ruled,vlined,linesnumbered]{algorithm2e}

\usepackage[mode=tex]{standalone} % mode=image|tex, mode=build, buildmissing


\usepackage{tikz}
% \usepackage{tkz-graph}

\usepackage{chronosys}
\usepackage{xspace}
\usetikzlibrary{shapes,arrows,calc,positioning,fit,automata}
\usetikzlibrary{decorations.markings}
\usetikzlibrary{overlay-beamer-styles}
\usepackage{fontawesome}

\usepackage{pgfplots}
\usepackage{pgfplotstable}
\usepackage{filecontents}

\usepackage{caption,subcaption}

\usepackage{soul}


\newcommand{\Xcal}{\mathcal{X}}
\newcommand{\Pcal}{\mathcal{P}}
\newcommand{\Qcal}{\mathcal{Q}}
\newcommand{\Mcal}{\mathcal{M}}
\newcommand{\Gcal}{\mathcal{G}}
\newcommand{\Fcal}{\mathcal{F}}
\newcommand{\Phat}{\hat{P}}
\newcommand{\Xhat}{\hat{X}}
\newcommand{\xhat}{\hat{x}}
\newcommand{\Ptilde}{\tilde P}
\newcommand{\ptilde}{\tilde p}
\newcommand{\E}{\mathbb{E}}
\newcommand{\funF}{\mathrm{f}}
\newcommand{\funC}{\mathrm{c}}
\newcommand{\funQ}{\mathrm{q}}
\newcommand{\funG}{\mathrm{g}}
\newcommand{\funD}{\mathrm{d}}
\newcommand{\funID}{\mathrm{id}}
\newcommand{\classL}{\mathrm{L}}

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}
\DeclareMathOperator*{\sgn}{sgn}


\newcommand{\define}{\triangleq}
\newcommand{\eps}{\varepsilon}
\newcommand{\transpose}{\intercal}
\newcommand{\dmin}{d_{\mathrm{min}}}
\newcommand{\mat}[1]{\ensuremath{\mathbf{#1}}}
\newcommand{\vect}[1]{\ensuremath{\mathbf{#1}}}
\newcommand{\sign}[1]{\mathrm{sgn}\left(#1\right)}
\newcommand{\Norm}[1]{\left\lVert#1\right\rVert}
\newcommand{\norm}[1]{||#1||}

\newcommand{\Pilots}{\mat{\tilde{X}}}
\newcommand{\pilots}{\vect{\tilde{x}}}

\newcommand{\NoiseQuant}{\mat{\delta Q}}
\newcommand{\noiseQuant}{\vect{\delta q}}
\newcommand{\NoisePilots}{\mat{Z}}
\newcommand{\noisePilots}{\vect{z}}


\newcommand{\myBlue}{blue!80!black}
\newcommand{\myGreen}{green!60!black}
\newcommand{\myRed}{red!80!black}


\newcommand{\Ndata}{N_\text{data}}
\newcommand{\Nsc}{N_\text{sc}}
\newcommand{\Nse}{N_\text{se}}
\newcommand{\Nfft}{N_\text{FFT}}
\newcommand{\Ptx}{P_\text{TX}}
\newcommand{\EBW}{\text{EBW}}
\newcommand{\ER}{\text{ER}}
\newcommand{\SNR}{\text{SNR}}
\newcommand{\SER}{\text{SER}}
\newcommand{\PAPR}{\text{PAPR}}



\newcommand{\noteRed}[1]{{\color{red}#1}}
\newcommand{\noteBlue}[1]{{\color{blue}#1}}


\newcommand{\Enc}{\mathrm{e}_\theta}
\newcommand{\Demod}{\mathrm{p}_\phi}
\newcommand{\Demodprime}{\mathrm{p}_\xi}
\newcommand{\SWEnc}{}
\newcommand{\SWDec}{}
\newcommand{\EntEnc}{}
\newcommand{\EntDec}{}
\newcommand{\EntMod}{\mathrm{q}_\zeta}


\definecolor{NYUviolet}{HTML}{57068c} 	% official NYU violet
\definecolor{NYUlight}{HTML}{8900e1} 	% NYU light violet
\definecolor{NYUdark}{HTML}{330662} 	% NYU dark violet
\definecolor{NYUnight}{HTML}{220337} 	% NYU darker violet



\newcommand\blfootnote[1]{%
	\begingroup
	\renewcommand\thefootnote{}\footnote{#1}%
	\addtocounter{footnote}{-1}%
	\endgroup
}


\newcommand{\algorithmsize}{\small}

%\newcommand{\note}[1]{{\color{red}#1}}
\newcommand{\ToDo}[1]{{\color{red}\textbf{\underline{#1}}}}
\newcommand{\highlight}[1]{{\bfseries#1}}
% \newcommand{\review}[1]{{\color{blue}#1}}
\newcommand{\review}[1]{{#1}}

\tikzstyle{block}=[rectangle,draw,very thick,fill=white,align=center,font=\Large]
\tikzstyle{edge} = [draw,very thick,->,-triangle 45]
\tikzstyle{plateBlue} = [draw=\myBlue, shape=rectangle, rounded corners=0.5ex, ultra thick,
minimum width=3.1cm, text=\myBlue, text width=3.1cm, align=right, inner sep=10pt, inner ysep=10pt,append after command={node[font=\bf,text=\myBlue,above left= 3pt of \tikzlastnode.south east] {#1}}]

\tikzstyle{plateRed} = [draw=\myRed, shape=rectangle, rounded corners=0.5ex, ultra thick,
minimum width=3.1cm, text=\myRed, text width=3.1cm, align=right, inner sep=10pt, inner ysep=10pt,append after command={node[font=\bf\LARGE,text=\myRed,above= 3pt of \tikzlastnode.south] {#1}}]


\tikzstyle{plateGreen} = [draw=\myGreen, shape=rectangle, rounded corners=0.5ex, ultra thick,
minimum width=3.1cm, text=green!80!black, text width=3.1cm, align=right, inner sep=10pt, inner ysep=10pt,append after command={node[font=\bf\LARGE,text=\myGreen,above= 3pt of \tikzlastnode.south] {#1}}]


\tikzstyle{plate} = [draw, shape=rectangle, rounded corners=0.5ex, ultra thick,
minimum width=3.1cm,  text width=3.1cm, align=right, inner sep=10pt, inner ysep=10pt,append after command={node[font=\bf\Large,above left= 3pt of \tikzlastnode.south east] {#1}}]


\tikzstyle{plateSmall} = [draw, shape=rectangle, rounded corners=0.5ex, ultra thick,
minimum width=3.1cm,  text width=3.1cm, align=right, inner sep=10pt, inner ysep=10pt,append after command={node[font=\bf,above= 3pt of \tikzlastnode.south] {#1}}]

\tikzstyle{plateUp} = [draw, shape=rectangle, rounded corners=0.5ex, ultra thick,
minimum width=3.1cm,  text width=3.1cm, align=right, inner sep=10pt, inner ysep=10pt,append after command={node[font=\bf\Large,above= 3pt of \tikzlastnode.north] {#1}}]

\tikzstyle{plateUpEast} = [draw, shape=rectangle, rounded corners=0.5ex, ultra thick,
minimum width=3.1cm,  text width=3.1cm, align=right, inner sep=10pt, inner ysep=10pt,append after command={node[font=\bf\Large,above= 3pt of \tikzlastnode.north east, anchor=south east] {#1}}]

\tikzstyle{plateDown} = [draw, shape=rectangle, rounded corners=0.5ex, ultra thick,
minimum width=3.1cm,  text width=3.1cm, align=right, inner sep=10pt, inner ysep=10pt,append after command={node[font=\bf\Large,below= 3pt of \tikzlastnode.south] {#1}}]


\usepackage[prefix=]{xcolor-material}
\pgfmathdeclarerandomlist{material}{%
	{Red}{Blue}{Green}}
\tikzset{%
	half clip/.code={
		\clip (0, -256) rectangle (256, 256);
	},
	color/.code=\colorlet{fill color}{#1},
	color alias/.code args={#1 as #2}{\colorlet{#1}{#2}},
	colors alias/.style={color alias/.list/.expanded={#1}},
	execute/.code={#1},
	on left/.style={.. on left/.style={#1}},
	on right/.style={.. on right/.style={#1}},
	split/.style args={#1 and #2}{
		on left ={color alias=fill color as #1},
		on right={color alias=fill color as #2, half clip}
	}
}
\newcommand\reflect[2][]{%
	\begin{scope}[#1]\foreach \side in {-1, 1}{\begin{scope}
				\ifnum\side=-1 \tikzset{.. on left/.try}\else\tikzset{.. on right/.try}\fi
				\begin{scope}[xscale=\side]#2\end{scope}
\end{scope}}\end{scope}}

\tikzset{%
	cat/.pic={
		\tikzset{x=1.5cm/5,y=1.5cm/5,shift={(0,-1/3)}}
		\useasboundingbox (-1,-1) (1,2);
		\fill [BlueGrey900] (0,-2)
		.. controls ++(180:3) and ++(0:5/4) .. (-2,0)
		arc (270:90:1/5)
		.. controls ++(0:2) and ++(180:11/4) .. (0,-2+2/5);
		\foreach \i in {-1,1}
		\scoped[shift={(1/2*\i,9/4)}, rotate=45*\i]{
			\clip [overlay] (0, 5/9) ellipse [radius=8/9];
			\clip [overlay] (0,-5/9) ellipse [radius=8/9];
			\fill [BlueGrey900] ellipse [radius=1];
			\clip [overlay] (0, 7/9) ellipse [radius=10/11];
			\clip [overlay] (0,-7/9) ellipse [radius=10/11];
			\fill [Purple100] ellipse [radius=1];
		};
		\fill [BlueGrey900] ellipse [x radius=3/4, y radius=2];
		\fill [BlueGrey100] ellipse [x radius=1/3, y radius=1];
		\fill [BlueGrey900]
		(0,15/8) ellipse [x radius=1, y radius=5/6]
		(0, 8/6) ellipse [x radius=1/2, y radius=1/2]
		{[shift={(-1/2,-2)}, rotate= 10]  ellipse [x radius=1/3, y radius=5/4]}
		{[shift={( 1/2,-2)}, rotate=-10] ellipse [x radius=1/3, y radius=5/4]};
		\fill [BlueGrey500]
		(-1/9,11/8) ellipse [x radius=1/5, y radius=1/5]
		( 1/9,11/8) ellipse [x radius=1/5, y radius=1/5];
		\fill [Purple100]
		(0,12/8)     ellipse [x radius=1/10, y radius=1/5]
		(0,12/8+1/9) ellipse [x radius=1/5 , y radius=1/10];
		\foreach \i in {-1,1}
		\scoped[shift={(1/2*\i,2)}, rotate=35*\i]{
			\clip [overlay] (0, 1/7) ellipse [radius=2/7];
			\clip [overlay] (0,-1/7) ellipse [radius=2/7];
			\fill [Yellow50] ellipse [radius=1];
		};
		\scoped{
			\clip (-1,-2) rectangle ++(2,1);
			\fill [BlueGrey900] (0,-2) ellipse [radius=1/2];
			\fill [Grey100]
			(-1/2,-2) ellipse [x radius=1/3, y radius=1/4]
			( 1/2,-2) ellipse [x radius=1/3, y radius=1/4];
		};
		\foreach \i in {-1,1}
		\foreach \j in {-1,0,1}
		\fill [Grey100, shift={(0,11/8)}, xscale=\i, rotate=\j*15,
		shift=(0:1/2)]
		ellipse [x radius=1/3, y radius=1/64];
	},
dog/.pic={
	\begin{scope}[x=1.5cm/480,y=1.5cm/480]
		\useasboundingbox (-256, -256) (256, 256);
		\reflect[split=Brown400 and Brown500]{
			\fill [fill color] (0,-64) ellipse [x radius=160, y radius=144];
			\fill [fill color] (0, 32) ellipse [x radius=128, y radius=112];
			\fill [fill color] (32,96)
			.. controls ++( 75:128) and ++(105:128) .. ++(192,  0)
			.. controls ++(285: 96) and ++(285: 96) .. ++(-80,-32)
			.. controls ++(105: 64) and ++( 75: 32) .. cycle;
		}
		\reflect[split={Grey100 and Grey200}]{
			\clip (0,-64) ellipse [x radius=160, y radius=144];
			\fill [fill color](0,-224) 
			.. controls ++(  0:64) and ++(270:64) .. ++(96,64)
			.. controls ++( 90:64) and ++(270:64) .. ++(-96,192)
			.. controls ++(270:64) and ++( 90:64) .. ++(-96,-192)
			.. controls ++(270:64) and ++(180:64) .. cycle;
		}
		\reflect[split={Pink100 and Pink200}]{
			\fill [fill color](0,-192) ellipse [x radius=28, y radius=32];
		}
		\reflect[split={BlueGrey800 and BlueGrey900}]{
			\fill [fill color](0,-144) 
			.. controls ++(  0:20) and ++(315:20) .. ++( 40,64)
			.. controls ++(135:20) and ++( 45:20) .. ++(-80, 0)
			.. controls ++(225:20) and ++(180:20) .. cycle;
			\fill [BlueGrey900] (56, 0) circle [radius=20];
			\fill [fill color] (-8,-112)
			-- ++(16,0) -- ++(0,-32) arc (180:360:24)
			arc (180:0:8) arc (360:180:40);
		}
\end{scope}}
}

\tikzset{
	o/.style={
		shorten >=#1,
		decoration={
			markings,
			mark={
				at position 1
				with {
					\draw circle [radius=#1];
				}
			}
		},
		postaction=decorate
	},
	o/.default=2pt
}




%% FROM https://tex.stackexchange.com/questions/103849/telecommunications-symbols


\tikzset{naming/.style={align=center,font=\large}}
\tikzset{antenna/.style={insert path={-- coordinate (ant#1) ++(0,0.25) -- +(135:0.25) + (0,0) -- +(45:0.25)}}}
\tikzset{station/.style={naming,draw,shape=dart,shape border rotate=90, minimum width=15mm, minimum height=30mm,outer sep=0pt,inner sep=3pt}}
\tikzset{stationPoster/.style={naming,draw,shape=dart,shape border rotate=90, minimum width=20mm, minimum height=40mm,outer sep=0pt,inner sep=3pt}}
%\tikzset{mobile/.style={naming,draw,shape=rectangle,minimum width=15mm,minimum height=7.5mm, outer sep=0pt,inner sep=3pt}}
\tikzset{mobile/.style={naming,draw,shape=rectangle,minimum width=12mm,minimum height=6mm, outer sep=0pt,inner sep=3pt}}
\tikzset{radiation/.style={{decorate,decoration={expanding waves,angle=90,segment length=4pt}}}}




\newcommand{\MBS}[1]{%
\begin{tikzpicture}
\node[station] (base) {#1};


\draw[line join=bevel] (base.100) -- (base.80) -- (base.120) -- (base.60) -- (base.mid west) -- (base.mid east);
\draw[line join=bevel] (base.mid east) -- (base.120) -- (base.60) (base.60) -- (base.100);

\draw[line cap=rect] ([xshift=-5mm,yshift=0mm]base.north -| base.right tail) [antenna=1];
\draw[line cap=rect] ([yshift=0mm]ant1 |- base.north) -- node[above,shape=rectangle,inner ysep=5]{\dots} ([xshift=5mm, yshift=0mm]base.north -| base.left tail) [antenna=2];

\end{tikzpicture}
}


\newcommand{\MBSposter}[1]{%
\begin{tikzpicture}
    \node[stationPoster] (base) {#1};
    
    \draw[line join=bevel] (base.100) -- (base.80) -- (base.120) -- (base.60) -- (base.mid west) -- (base.mid east);
    \draw[line join=bevel] (base.mid east) -- (base.120) -- (base.60) (base.60) -- (base.100);
    
    \draw[line cap=rect] ([xshift=-5mm,yshift=0mm]base.north -| base.right tail) [antenna=1];
    \draw[line cap=rect] ([yshift=0mm]ant1 |- base.north) -- node[above,shape=rectangle,inner ysep=5]{\scriptsize\dots} ([xshift=5mm, yshift=0mm]base.north -| base.left tail) [antenna=2];

\end{tikzpicture}
}


==> figures/data/BPSK_Ours_v9_tested_var_0.1.tex <==
X	Y
% X: SNR (P_x / sigma_n^2)
% Y: log10(SER/BER)


#-72.45387495602819	-0.30094635486602783
#-66.88001311350692	-0.30087512731552124
0.06699859736026645	-0.7679653167724609
1.5657485927931678	-0.8947674632072449
2.4277744060547684	-0.9856747984886169
3.445485070027241	-1.112034559249878
4.139842677518955	-1.2144335508346558
4.629231871610351	-1.2980729341506958
5.000942476272038	-1.3689827919006348
5.280262194491324	-1.41788911819458
#5.53929550077109	-1.476643681526184
5.737192290464305	-1.5187468528747559
#5.935344752954935	-1.5629299879074097
#6.07497126931807	-1.5953266620635986
#6.254158938316264	-1.6421293020248413
6.309730958598449	-1.6461082696914673
#6.4681860674	-1.6781575680
6.5482820742	-1.7035191059
#6.6320652185	-1.7298754454
#6.8103556933	-1.7948255539
#6.8236382358	-1.7750872374
#6.9636484024	-1.8192574978
7.0258722747	-1.8413929939
#7.1337153076	-1.8611531258
7.2545799477	-1.9002234936
#7.3539704969	-1.9322159290
#7.4083961801	-1.9337776899
#7.6186166782	-2.0416896343
#7.5940959290	-2.0123407841
7.7208180702	-2.0529117584

==> figures/data/BPSK_Ours_v9_tested_var_0.5.tex <==
X	Y
% X: SNR (P_x / sigma_n^2)
% Y: log10(SER/BER)


#-74.13749140793391	-0.3009032905101776
#-68.04248585947256	-0.30101510882377625
0.5092199954409252	-0.7390666007995605
2.0376966725309646	-0.8689849376678467
2.897319396884664	-0.9668225646018982
3.8819679927244337	-1.0973403453826904
4.535399088275191	-1.2001160383224487
5.013112803802225	-1.2926522493362427
5.373684966133586	-1.363620638847351
5.632078712665136	-1.412287950515747
#5.879035413455119	-1.4683942794799805
6.05277344967466	-1.5086631774902344
#6.248822860514696	-1.549425721168518
6.389997224760565	-1.5875827074050903
#6.557085073534755	-1.636067271232605
6.624677771474992	-1.647706389427185
#6.7528892132	-1.6707980633
#6.8470663472	-1.6937317848
6.9225705822	-1.7223365307
#7.0915757143	-1.7909948826
#7.1037799307	-1.7655204535
# 7.2323298402	-1.8035373688
#7.2936142135	-1.8377859592
7.3968137632	-1.8479969501
#7.5045635634	-1.8950536251
#7.6055833130	-1.9287220240
7.6573756598	-1.9287220240
#7.8592745130	-2.0283560753
#7.8489743102	-2.0073413849
7.9508176203	-2.0452141762

==> figures/data/BPSK_Ours_v9_tested_var_1.0.tex <==
X	Y
% X: SNR (P_x / sigma_n^2)
% Y: log10(SER/BER)


#-75.01571034042516	-0.30177783966064453
#-68.56223635230253	-0.30065491795539856
0.7706805625178431	-0.7151798009872437
2.3538834683562113	-0.8499100208282471
3.2401462366863343	-0.9441742897033691
4.237282539569495	-1.0769224166870117
4.897356657065357	-1.1791778802871704
5.3775311795337295	-1.2714977264404297
5.715979950742296	-1.343796730041504
5.96510949086992	-1.387040615081787
#6.215047356913306	-1.4496136903762817
6.389591997808689	-1.491297960281372
#6.584692224547844	-1.5279792547225952
6.713734119180833	-1.5675569772720337
6.879376749825625	-1.6159886121749878
#6.951510758614213	-1.6120548248291016
#7.0706245610	-1.6530017853
#7.1648367435	-1.6721003056
7.2322852967	-1.6964204311
#7.4051790125	-1.7713282108
#7.4079347801	-1.7366431952
#7.5204768211	-1.7887991667
7.5890625248	-1.8219978809
#7.6972225597	-1.8154226542
#7.7892407040	-1.8680975437
7.8884043817	-1.9078608751
#7.9452135758	-1.8977944851
8.1365386996	-2.0090720654
#8.1346464580	-1.9722360373
8.2276136266	-2.0258870125

==> figures/data/QPSK_Ours_other.tex <==
X	Y
% X: SNR (P_x / sigma_n^2)
% Y: log10(SER/BER)
% Structured Ps = 1.5, Sinusoid

-1.2461081761	-0.3626916409
1.073842521	-0.5304054022
1.5762859428	-0.5775294900
2.8612794489	-0.6403489113
4.2530266814	-0.7425371408
5.1421191254	-0.8875051141
6.1208055261	-1.0832575560 
6.7130288993	-1.2234432697
7.0413401520	-1.3182641268 
7.6156651363	-1.4907847643
7.9728758418	-1.6044088602 
8.5052419641	-1.7996815443
8.8142719732	-1.9225795269
9.2440899141	-2.1109368801
9.7285042061	-2.3458306789 
10.2926782348	-2.6467688084 
11.1077338372	-3.1392152309
11.8532538506	-3.6569879055 
12.7903979345	-4.5582017899 





==> figures/data/QPSK_Ours_other2.tex <==
X	Y
% X: SNR (P_x / sigma_n^2)
% Y: log10(SER/BER)
% Structured Ps = 4.5, Leaky Relu

-0.2082543415	-0.5208468437
1.3601956670	-0.6408811808
2.3116056860	-0.7358895540
2.9692819426	-0.8140546679
3.5509495245	-0.8860785961
3.8576119881	-0.9273463488
4.4529373091	-1.0184683800
5.0139650366	-1.0359466076
5.6739331579	-1.1620868444
6.4549881696	-1.3415355682
7.1195651500	-1.4707112503
7.7373765707	-1.6413307190
8.1032888678	-1.7587187290
8.8249539165	-2.0403237343
9.2138073460	-2.1924557686

==> figures/data/QPSK_Ours_v8_tested_var_0.1.tex <==
X	Y
% X: SNR (P_x / sigma_n^2)
% Y: log10(SER/BER)

# -63.33259337377928	-0.12496911734342575
# -58.94368295311867	-0.12516522407531738
# -54.67096336912934	-0.12543217837810516
-0.4176885520543894	-0.47401162981987
0.6590820883245753	-0.5445454716682434
1.392003213477706	-0.6023881435394287
# 2.460180146893751	-0.6502423286437988
2.9686234208119844	-0.7029585838317871
# 2.897046039470395	-0.7592918276786804
# 4.186460585118961	-0.7684972286224365
# 4.433091609390982	-0.8902758359909058
4.606028229128279	-0.9240444302558899
# 4.943223255411758	-0.9640876650810242
 5.168593818044213	-1.012532353401184
# 5.703070852145653	-0.9835401177406311
# 5.558040272201281	-1.0749000310897827
5.68314678190414	-1.1139578819274902
# 5.8430689112332335	-1.1532326936721802
#5.51083410509368	-1.144151210784912
# 6.478678962849381	-1.2481168508529663
6.318563897351942	-1.2689975500106812
# 6.578331521465307	-1.3153094053268433
6.662708134294922	-1.3740003108978271
# 6.994790128370764	-1.4150041341781616
# 6.995158256212312	-1.4229158163070679
# 7.0834010762525015	-1.4493454694747925
7.419522944254856	-1.5650851726531982
# 7.674630485846759	-1.5932600498199463
# 7.824079503397377	-1.662170171737671
7.822014777421731	-1.6881210803985596

==> figures/data/QPSK_Ours_v8_tested_var_0.5.tex <==
X	Y
% X: SNR (P_x / sigma_n^2)
% Y: log10(SER/BER)

# -64.5869415100635	-0.1250348538160324
# -59.65996510670789	-0.1253962367773056
# -55.82464510621031	-0.12514255940914154
-0.07673278723952351	-0.440672367811203
1.0707652991149321	-0.5178601741790771
1.8442083283851547	-0.5782879590988159
# 2.6819861064868284	-0.620784342288971
3.204025051574322	-0.6768074631690979
# 3.335230537961026	-0.741387128829956
# 4.203603583883661	-0.7267138957977295
# 4.685005813060635	-0.8644477128982544
4.8220527923560015	-0.8760039210319519
# 5.127002639933696	-0.9092063307762146
5.369857563287603	-0.9599058628082275
# 5.61442191101248	-0.8894016742706299
5.7117517104155855	-1.0078048706054688
# 5.9315532267038185	-1.0743049383163452
# 6.0951470981942215	-1.1180368661880493
# 5.978151632828292	-1.1436896324157715
# 6.642215230809229	-1.1798667907714844
6.703126486763528	-1.2705546617507935
# 6.850873774736739	-1.2832084894180298
6.9366328163709845	-1.353193759918213
# 7.2046651115412015	-1.3735203742980957
# 7.224500742878525	-1.3814423084259033
# 7.312878661634453	-1.4201281070709229
7.64986553627554	-1.542871117591858
# 7.880336385363823	-1.5553064346313477
8.041579962232197	-1.6476879119873047
# 7.98688145363041	-1.67377769947052

==> figures/data/QPSK_Ours_v8_tested_var_1.0.tex <==
X	Y
% X: SNR (P_x / sigma_n^2)
% Y: log10(SER/BER)

# -65.27913272038022	-0.12479020655155182
# -60.25458896710298	-0.1252475529909134
# -56.12598486392484	-0.12509119510650635
0.038661993904185156	-0.4134184420108795
1.282374361942701	-0.4882698655128479
2.0995471450168597	-0.5522392988204956
# 2.8091697228211823	-0.6015930771827698
3.341449588690853	-0.656197190284729
# 3.651090501387531	-0.7122980952262878
# 4.201848230248	-0.7177929878234863
4.842527590078863	-0.8461679220199585
# 4.912062740457269	-0.8291041851043701
# 5.2639468809015035	-0.8768982887268066
5.520161954862862	-0.9308289885520935
# 5.616812377228335	-0.8771666288375854
5.863882220491851	-0.9753669500350952
# 6.09810820658487	-1.042899250984192
# 6.26770971069957	-1.0924090147018433
# 6.214210872473453	-1.0791829824447632
# 6.771019844717106	-1.138530969619751
6.890333730832618	-1.2129566669464111
# 7.034649667418044	-1.237497091293335
7.156760081050018	-1.305633544921875
# 7.364114598296979	-1.327347993850708
# 7.398883372463871	-1.336643934249878
# 7.489468462816208	-1.377730131149292
# 7.848014827848981	-1.4929572343826294
8.063283647273972	-1.4868661165237427
8.250758289443983	-1.6024645566940308
8.216918303130226	-1.6443880796432495
